Complex Knowledge Base Question Answering: A Survey

Knowledge base question answering (KBQA) aims to answer a question over a knowledge base (KB). Early studies mainly focused on answering simple questions over KBs and achieved great success. However, their performance on complex questions is still far from satisfactory. Therefore, in recent years, researchers propose a large number of novel methods, which looked into the challenges of answering complex questions. In this survey, we review recent advances on KBQA with the focus on solving complex questions, which usually contain multiple subjects, express compound relations, or involve numerical operations. In detail, we begin with introducing the complex KBQA task and relevant background. Then, we describe benchmark datasets for complex KBQA task and introduce the construction process of these datasets. Next, we present two mainstream categories of methods for complex KBQA, namely semantic parsing-based (SP-based) methods and information retrieval-based (IR-based) methods. Specifically, we illustrate their procedures with flow designs and discuss their major differences and similarities. After that, we summarize the challenges that these two categories of methods encounter when answering complex questions, and explicate advanced solutions and techniques used in existing work. Finally, we conclude and discuss several promising directions related to complex KBQA for future research.

==> back.tex <==

\section{Background}
\label{sec:task_dataset}
%In this section, we first give a task definition about complex KBQA. 
In this section, we first give a task definition about complex KBQA, and then introduce available  datasets for this task.
% with respects to the main factors in complex questions.
% Then, we illustrate~\glcomment{Is there a better description?} the complex question types with existing datasets and introduce other factors to consider when constructing complex KBQA datasets.
% ~\yscomment{We can indicate that we group them by the main factors. ``we introduce available complex KBQA datasets with respects to the main factors in complex questions.''}
%Then, we introduce available complex KBQA datasets with respect to the main factors in complex questions.
 % different question types with categorization of existing datasets.
% Next, we present an overview of existing benchmarks for this task.
% The statistics summary of these datasets is shown in Tab.~\ref{tab:datasets}.

%\subsection{Task Definition}
\ignore{
Formally speaking, a KB consists of a set of facts, where the subject and object are connected by their relation.
All the subjects and objects in facts form the entity set of the KB.
A complex question is a natural language question which is in the format of a sequence of tokens.
We define the complex KBQA task as follows.
Given a question and an associated KB, the system is supposed to retrieve the entities or aggregate the retrieved entities from the entity set as the corresponding answers.
Generally, the ground truth answers of the questions are provided to train a complex KBQA system.
}
\subsection{What is KBQA}. For the task of complex KBQA, a KB consisting of a set of facts is given as input, where the subject and object are connected by their relation. 
%Formally speaking, a KB consists of a set of facts, where the subject and object are connected by their relation.
All the subjects and objects in the facts form the entity set of a KB.
Given the available  KB, this task aims to answer complex natural language questions in the format of a sequence of tokens. 
% ~\cite{CWQ-NAACL-2018}.~\glcomment{How about deleting the citation?} 
Specially, we assume the correct answers come from the entity set of the KB. 
Unlike answers of simple KBQA task, which are entities directly connected to the topic entity, the answers of the complex KBQA task are entities multiple hops away from the topic entities or even the aggregation of them.
%A complex question is a natural language question which is in the format of a sequence of tokens. 
% As introduced in Section~\ref{sec:intro}, complex questions contain some queries that are not involved in the simple questions, namely multi-hop reasoning or constrained relations or numerical operations.~\yscomment{I don't think we need to repeat this to highlight complex KBQA.}
%We define the complex KBQA task as follows.
% Given a complex question and an associated KB, the system is supposed to retrieve the entities or aggregate the retrieved entities from the entity set as the corresponding answers.
%Given a question and an associated KB, the system is supposed to predict correct answers.
%Unlike answers of simple KBQA task, which are entities directly connected to the topic entity, the answers of the complex KBQA task are entities multiple hops away from the topic entities or even the aggregation of them.
% Unlike simple KBQA task, where the answers are entities directly connected to the topic entity, the answers of complex KBQA could be entities multiple hops away from the topic entities in the KB or even the aggregation of entities.~\glcomment{Unlike simple KBQA task, where the answers are entities directly connected to the topic entity, the complex KBQA task usually require to return entities multiple hops away from the topic entities or even the aggregation of entities.
% conduct multi-hop reasoning on KB to obtain answers or involve further aggregation to deal with constraints and numerical questions.}
% ~\glcomment{Do you think we should add one sentence to describe "To solve complex questions, more operations (complex methods) are introduced to tackle with query complexity."}
% ~\jhcomment{the complex KBQA system is trained with only the ground truth answers of the questions provided?}

\subsection{Evaluation Protocol }

\subsection{Traditional approaches for simple KBQA}

==> sec-app.tex <==
\begin{sidewaystable*}[htbp]
\addtolength{\tabcolsep}{-1.8pt} 
	\centering
	\caption{Statistic of different methods \yscomment{Should we include the publish years of these methods.}}
    % ~\glcomment{We may also include pipeline stage here as a column}}
    % \begin{scriptsize}
	\begin{tabular}{c | c c c c c c c c c c c c c | c}
		\hline
		Methods & WQ & CQ & WQSP & CWQ & QALD & LQ & LQ2 & MQA-1h & MQA-2h & MQA-3h & CFQ & GQA & KQA & CODE \\
		\hline
        \cite{Yih-ACL-2015} & 52.5(F1) & - & - & - & - & - & - & - & - & - & - & - & - &\href{https://aclanthology.org/P15-1128.pdf}{url}\\
        \cite{Bast-CIKM-15} & 49.4(F1) & - & - & - & - & - & - & - & - & - & - & - & - &\href{https://ad-publications.cs.uni-freiburg.de/freebase-qa.pdf}{url}\\
        \cite{Yih-ACL-2016} & - & - & 66.8(F1) & - & - & - & - & - & - & - & - & - & - &\href{https://aclanthology.org/P16-2033.pdf}{url}\\
		\cite{Abujabal-WWW-17} & 51.0(F1) & 49.2(F1) & - & - & - & - & - & - & - & - & - & - & - & \href{http://papers.www2017.com.au.s3-website-ap-southeast-2.amazonaws.com/proceedings/p1191.pdf}{url}\\
		\cite{Liang-ACL-17} & - & - & 69.0(F1) & - & - & - & - & - & - & - & - & - & - &\href{https://arxiv.org/pdf/1611.00020.pdf}{url}\\
		\cite{Hu-EMNLP-18} & 53.6(F1) & 54.3(F1) & - & - & - & - & - & - & - & - & - & - & - &\href{https://aclanthology.org/D18-1234.pdf}{url}\\
		\cite{Luo-EMNLP-2018}& 52.7(F1) & 42.8(F1) & - & - & - & - & - & - & - & - & - & - & - &\href{https://aclanthology.org/D18-1242.pdf}{url}\\
		\cite{Jia-CIKM-2018} & - & - & - & - & - & - & - & - & - & - & - & - & - &\href{https://arxiv.org/pdf/1908.03650.pdf}{url}\\
		\cite{Abujabal-WWW-2018}& 51.0(F1) & - & - & - & - & - & - & - & - & - & - & - & - &\href{https://myahya.org/publications/neqa-abujabal-www2018.pdf}{url}\\
        \cite{Zafar-ESWC-2018} & - & - & - & - & - & 75.0(F1) & - & - & - & - & - & - & - &\href{http://jens-lehmann.org/files/2018/eswc_qa_query_generation.pdf}{url}\\
        \cite{Zheng-VLDB-2018} & 62.0(F1)& 71.0(F1) & - & - & - & - & - & - & - & - & - & - & - &\href{https://www.ccs.neu.edu/home/vip/teach/IRcourse/10_QA/p1373-zheng.pdf}{url}\\
        \cite{Hu-TKDE-2018} & - & - & - & - & - & - & - & - & - & - & - & - & - &\href{https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8085196}{url}\\
		\cite{Chen-NAACL-2019}& - & - & 82.6(A) & - & - & - & - & - & - & - & - & - & - &\href{https://arxiv.org/pdf/1904.01246.pdf}{url}\\
		\cite{Saha-TACL-2019}& - & - & 82.9(F1) & - & - & - & - & - & - & - & - & - & - &\href{https://aclanthology.org/Q19-1012.pdf}{url}\\
		\cite{Bhutani-CIKM-2019} & - & - & 60.3(F1) & 33.9(F1) & - & - & - & - & - & - & - & - & - &\href{https://dl.acm.org/doi/pdf/10.1145/3357384.3358033}{url}\\
		\cite{Lan-ICDM-2019}& - & - & - & - & - & - & - & 98.1(F1) & - & - & - & - & - &\href{https://ink.library.smu.edu.sg/cgi/viewcontent.cgi?article=5939&context=sis_research}{url}\\
        \cite{Maheshwari-ISWC-2019}& - & - & - & - & - & 71.0(F1) & - & - & - & - & - & - & - &\href{https://arxiv.org/pdf/1811.01118.pdf}{url}\\
        \cite{Zhu-Neuro-2020}& 52.1(F1) & - & 63.7(F1) & - & - & - & - & - & - & - & - & - & - &\href{https://www.sciencedirect.com/science/article/pii/S0925231219312639}{url}\\
		\cite{Skeleton-AAAI-2020}& - & - & - & 31.6(P1) & - & - & - & - & - & - & - & - & - &\href{https://arxiv.org/pdf/2003.13956.pdf}{url}\\
		\cite{Chen-IJCAI-2020}& 53.4(F1) & 43.1(F1) & - & - & - & 74.8(F1) & - & - & - & - & - & - & - &\href{https://www.ijcai.org/proceedings/2020/0519.pdf}{url}\\
		\cite{Lan-ACL-2020}& - & 43.3(F1) & 74.0(F1) & 40.4(F1) & - & - & - & - & - & - & - & - & - &\href{https://aclanthology.org/2020.acl-main.91.pdf}{url}\\
		\cite{Hua-JWS-2020}& - & - & 72.0(F1) & - & - & - & - & - & - & - & - & - & - &\href{https://arxiv.org/pdf/2010.15881.pdf}{url}\\
		\cite{Qiu-CIKM-2020}& 54.8(F1) & 45.0(F1) & - & - & - & - & - & - & - & - & - & - & - &\href{https://dl.acm.org/doi/pdf/10.1145/3340531.3411888}{url}\\
		\cite{Kapanipathi-AAAI-2021}& - & - & - & - & - & 44.5(F1) & - & - & - & - & - & - & - &\href{https://dl.acm.org/doi/pdf/10.1145/3336191.3371812}{url}\\
        \hline
		\hline
		\cite{KVMem-EMNLP-2016}& - & - & 46.7(A) & 21.1(A) & - & - & - & 96.2(A) & 82.7(A) & 48.9(A) & - & - & - &\href{https://arxiv.org/pdf/1606.03126.pdf}{url}\\
		\cite{Zhang-AAAI-2018}& - & - & - & - & - & - & - & 97.5(A) & 89.9(A) & 62.5(A) & - & - & - &\href{https://arxiv.org/pdf/1709.04071.pdf}{url}\\
		\cite{Zhou-COLING-2018}& - & - & - & - & - & - & - & - & - & - & - & - & - &\href{https://arxiv.org/pdf/1801.04726.pdf}{url}\\
		\cite{Sun-EMNLP-2018}& - & - & 66.4(A) & 32.8(A) & - & - & - & 97.0(A) & 94.8(A) & 77.7(A) & - & - & - &\href{https://arxiv.org/pdf/1809.00782.pdf}{url}\\
		\cite{Xiong-ACL-2019}& - & - & 67.2(A) & - & - & - & - & - & - & - & - & - & - &\href{https://aclanthology.org/P19-1417.pdf}{url}\\
		\cite{Sun-EMNLP-2019}& - & - & 68.1(A) & 45.9(A) & - & - & - & 97.0(A) & 99.9(A) & 91.4(A) & - & - & - &\href{https://arxiv.org/pdf/1904.09537.pdf}{url}\\
		\cite{Xu-NAACL-2019}& 54.6(F1) & - & - & - & - & - & - & - & - & - & - & - & - &\href{https://aclanthology.org/N19-1301.pdf}{url}\\
		\cite{Han-IJCAI-2020}& - & - & - & - & - & - & - & 98.8(A) & 93.7(A) & - & - & - & - &\href{https://www.ijcai.org/proceedings/2020/0500.pdf}{url}\\
		\cite{Apoorv-ACL-2020}& - & - & 66.6(A) & - & - & - & - & 97.5(A) & 98.8(A) & 94.8(A) & - & - & - &\href{https://aclanthology.org/2020.acl-main.412.pdf}{url}\\
		\cite{Han-EMNLP-2020}& - & - & 68.4(A) & - & - & - & - & - & - & - & - & - & - &\href{https://aclanthology.org/2020.findings-emnlp.133.pdf}{url}\\
		\cite{Qiu-WSDM-2020}& - & - & - & - & - & - & - & 97.0(A) & 95.1(A) & 75.2(A) & - & - & - &\href{https://dl.acm.org/doi/pdf/10.1145/3336191.3371812}{url}\\
		\cite{He-WSDM-2021}& - & - & 74.3(A) & 48.8(A) & - & - & - & 97.3(A) & 99.9(A) & 98.9(A) & - & - & - &\href{https://arxiv.org/pdf/2101.03737.pdf}{url}\\
		\cite{Feng-EMNLP-2021}& - & - & 68.6(A) & 47.4(A) & - & - & - & - & - & - & - & - & - &\href{https://aclanthology.org/2021.findings-emnlp.159.pdf}{url}\\
		\cite{Zhang-arxiv-2022}& - & - & 83.2(A) & 58.4(A) & - & - & - & - & - & - & - & - & - &\href{https://arxiv.org/pdf/2202.13296.pdf}{url}\\
		\hline
	\end{tabular}%
% 	\end{scriptsize}
    \label{tab:statistic}
\end{sidewaystable*}%

==> sec-data.tex <==
\ignore{
\begin{table}[!tbp]
    %\fontsize{3pt}{3pt}\selectfont
	\centering
	\caption{Several KBQA benchmark datasets involving complex questions. ``\textbf{LF}" denotes whether the dataset provides \textbf{L}ogical \textbf{F}orms, ``\textbf{NL}" denotes whether the dataset incorporates crowd workers to rewrite questions in \textbf{N}atural \textbf{L}anguage.
% 	and "\textbf{NU}" denotes whether the dataset contains the questions which require \textbf{NU}merical operations.
% 	"\textbf{CO}" denotes whether the dataset contains questions with \textbf{CO}nstraints, 
	%\yscomment{LC-QuAD 2.0 occupies two rows but it's unclear without the table border; Can we include a column to inidcate ``multi-hop reasoning'' property; Some cells are empty? The author of QALD?}~\glcomment{How about using hline to separate these datasets. Later, we should check all attributes again.}
	}
	\label{tab:datasets}%
% 	\begin{footnotesize}
	\begin{scriptsize}
% 	\setlength{\tabcolsep}{1mm}{
	\begin{tabular}{c | c c c c}
		%\cline{3-7}
		\hline
		% \multirow{2}{*}{Datasets}	&	\multirow{2}{*}{Reference}&	\multirow{2}{*}{KB\\Source}&	\multirow{2}{*}{Size}&	\multirow{2}{*}{Logical\\forms}& \multirow{2}{*}{Reasoning\\depth}& \multirow{2}{*}{Constraints}\\
% 		\multicolumn{2}{c|}{\multirow{2}{*}{\tabincell{c}{Datasets}}}
		\multirow{2}{*}{Datasets}&	\multirow{2}{*}{KB}&	\multirow{2}{*}{Size}&	\multirow{2}{*}{LF}& \multirow{2}{*}{NL}\\
		% \multirow{2}{*}{Datasets}	&	KB&	\multirow{2}{*}{Size}&	Logical&	Reasoning&	With & Manual\\
% 		\multirow{2}{*}{Datasets}
			&	&	&	&	\\
		\hline
		\hline
		% MetaQA-1hop	&	\cite{Zhang-AAAI-2018}&	MetaQA&	116,045&	No&	1&	No&	No\\
		% MetaQA-2hop	&	\cite{Zhang-AAAI-2018}&	MetaQA&	148,724&	No&	2&	No&	No\\
		% MetaQA-3hop	&	\cite{Zhang-AAAI-2018}&	MetaQA&	142,744&	No&	3&	No&	No\\
		WebQuestions~\cite{Berant-EMNLP-2013}&	Freebase&	5,810&	No&	\gladd{No}\\
		ComplexQuestions~\cite{Bao-COLING-2016}&	Freebase&	2,100&	No&	No\\
		WebQuestionsSP~\cite{Yih-ACL-2016}&	Freebase&	4,737&	Yes&	Yes\\
% 		ComplexWebQuestions~\cite{CWQ-NAACL-2018}&	Freebase&	34,689&	Yes&	Yes&	Yes&	Yes\\
        ComplexWebQuestions&	\multirow{2}{*}{Freebase}&	\multirow{2}{*}{34,689}&	\multirow{2}{*}{Yes}&	\multirow{2}{*}{Yes}\\
		\cite{CWQ-NAACL-2018}&	&	&	&\\
		\hline
		QALD series~\cite{QALD}&	DBpedia&	-&	Yes&	Yes\\
		LC-QuAD~\cite{LC-QuAD-ISWC-2017}&	DBpedia&	5,000&	Yes&	Yes\\
		\multirow{2}{*}{LC-QuAD 2.0~\cite{LC-QuAD-2.0-ISWC-2019}}&	\multirow{2}{*}{\tabincell{c}{DBpedia,\\Wikidata}}&	\multirow{2}{*}{30,000}&	\multirow{2}{*}{Yes}&	\multirow{2}{*}{Yes}\\
		&	&	&	&\\
		\hline
		MetaQA	Vanilla~\cite{Zhang-AAAI-2018}&	WikiMovies&	400k&	No&	No\\
		CFQ~\cite{CFQ-ICLR-2020}& Freebase&	239,357&	Yes&	No\\
		GrailQA~\cite{GrailQA-2020}&	Freebase&	64,331&	Yes&Yes\\
		KQA Pro~\cite{KQA-Pro}&	Wikidata&	117,970&	Yes&	Yes\\
		\hline
	\end{tabular}%
% 	}
% 	\end{footnotesize}
	\end{scriptsize}
\end{table}%
}

\section{Datasets}
\label{sec:data}
% Generally, the answers of the questions should be provided to train a complex KBQA system. ~\yscomment{I feel this sentence is not informative, how about use your previous version ``Over the decades, many efforts have been devoted to constructing datasets for complex KBQA.''}
Over the decades, much effort has been devoted to constructing datasets for complex KBQA. 
% For this purpose, many efforts have been devoted to constructing datasets for complex KBQA. ~\yscomment{We can remove the first sentence? how about ``Over the decades, many efforts ...''}
We list the available  complex KBQA datasets in Table~\ref{tab:datasets}.
%\yscomment{I'm rethinking the re-arganization of the paper, would it be better if we talk about Approaches first?}
% In this section, we take a brief introduction to existing complex KBQA datasets.~\yscomment{Could illustrate a little bit more. As the readers would already know that we are going to talk about the dataset from the last sentence in the last paragraph. We can introduce more about the organization of this section.}
% Tab.~\ref{tab:datasets} shows some attributes of complex KBQA datasets, including its scale, features and annotation situation.
% There have been a number of datasets collected for the complex KBQA task. 
% In this section, we first present the properties of complex questions of these datasets and then describe datasets in detail. 
% The statistics summary of datasets is shown in Table~\ref{tab:datasets}.~\glcomment{Is there a better organization of this paragraph? And you can check whether we need describe "natural language" and  "logic form" factors. As the two factors are labled in Table~\ref{tab:datasets}}~\yscomment{Could it be better to mention that we have the statistics at the end of the section?}
% ~\glcomment{I comment the complex dataset properties out. After yunshi modify the introduction part, I'll try to add it to introduction part.}
In order to serve realistic applications, these datasets typically contain questions which require multiple KB facts to reason. Moreover, they might include numerical operations (\eg counting and ranking operations for comparative and superlative questions, respectively) and constraints (\eg entity and temporal keywords), which further increase the difficulty in reasoning the answers from KBs.

Overall, these datasets are constructed with the following steps: Given a topic entity in a KB as a question subject, simple questions are first created with diverse templates. Based on simple questions and neighborhood of topic entities in a KB, complex questions are further generated with predefined composition templates, 
% ~\yscomment{To avoid confusion of above two ``tempaltes'', how about ``predefined composition templates''?}, 
and another work~\cite{KQA-Pro} also generates executable logic forms with templates. 
Meanwhile, answers are extracted with corresponding rules. 
% In some cases, crowd workers are hired to paraphrase the template queries into natural language questions~\yscomment{can we remove the content ``the template queries ... questions'' as the templates should also be natural language questions.}~\glcomment{template-based or machine-generated questions.} 
In some cases, crowd workers are hired to paraphrase the canonical questions, 
% into more natural forms~\cite{GrailQA-2020}~\yscomment{How about changing ``into more natural forms'' to ``for the creation of more varied and fluent text''}~\glcomment{To discuss}, 
and refine the generated logic forms, making the question expressions more diverse and fluent. 
% In order to serve realistic applications, these datasets typically create questions which require multiple KB facts to reason. 
% for diverse intensions~\yscomment{What do you mean by ``diverse intensions''?}
% For example, deriving from \textbf{WebQuestions} dataset, where most questions only require single fact reasoning on KB, \textbf{ComplexQuestions} dataset incorporated entity type, and temporal constraints to form complex questions.

%Different from simple questions which don't involve multi-hop reasoning on KB, most of complex KBQA datasets contain questions which require multiple KB facts to reason. Moreover, complex questions involves numerical operations (\eg counting, ranking operations for comparative or superlative questions) and constraints (entity, temporal keywords), which further increase the difficulty to reason answers from KBs. Compared with template based generated queries, human's paraphrasing makes it more difficult to understand complex questions in diversified expression.

\ignore{
% As introduced in Sec.~\ref{sec:intro}, there are three complex question types: questions involving \emph{multi-hop} reasoning or \emph{constrained} relations or \emph{numerical} operations. 
As introduced in Section~\ref{sec:intro}, complex questions contain some queries that are not involved in the simple questions, namely 
% questions involving ~\jhcomment{delete "questions involving"?}
multi-hop reasoning or constrained relations or numerical operations.
Complex questions involve constraints (entity, temporal keywords), which indicates we need to consider some constrained relations to get answers.  
% ~\yscomment{We don't need to emphasis these factors here as we have done in the Introduction Section.}
For example, deriving from \textbf{WebQuestions} dataset, where most questions only require single fact reasoning on KB, \textbf{ComplexQuestions} dataset incorporated entity type, and temporal constraints to form complex questions.
Different from simple questions which which don't involve multi-hop reasoning on KB
% ~\yscomment{To avoid repeating above sentence, we can say ``which don't involve multi-hop reasoning on KB''}
, most of complex KBQA datasets contain questions which composite multiple KB facts to reason.
% This type of question is called question involve \emph{multi-hop} reasoning. 
Such questions can be easily generated by composition rules (\eg \textbf{MetaQA Vanilla} and \textbf{CFQ}). 
Moreover, complex questions involve numerical operations (\eg counting, ranking operations for comparative or superlative questions). % require further answer aggregation. 
% As shown in Table~\ref{tab:datasets} , 
Most of complex KBQA benchmarks (\eg \textbf{WebQuestionsSP} and \textbf{ComplexWebQuestions}) include questions of such type.
%~\yscomment{Why above descriptions to the complex factors are splitted into two paragraphs?}
% To obtain answer for question in  Fig,~\ref{fig:example}, we should rank all possible candidates according to their marriage date after a series of reasoning steps to fullfill the constraint ``first''.
%~\yscomment{``Deriving from \textbf{WebQuestions} dataset, where most questions only require single fact reasoning on KBs, \textbf{ComplexQuestions} dataset incorporates entity type, and temporal constraints to form complex questions.''}

Besides different complex queries, some other factors are taken into consideration when constructing the complex KBQA datasets .
Compared with questions generated with templates, natural language questions written by humans are more challenging to answer. 
For example, complex questions in \textbf{QALD}, \textbf{LC-QuAD 1.0} and \textbf{LC-QuAD 2.0} datasets are paraphrased by crowd workers after template based generation. 
As manually annotating complex questions with specific logic forms is expensive and labor-intensive, some existing datasets (\eg \textbf{GrailQA} and \textbf{KQA Pro}) adopt off-the-shelf logical form generation algorithms or predefined rules to generate logical forms.
% Complex question can be transformed into specific logic form $l$ (\eg SPARQL, query graph) with the consideration of the structured KBs. Recent released datasets \textbf{GrailQA} and \textbf{KQA Pro} adopt the existing logical form generation algorithm or predefined rules to generate logical forms.
}

\ignore{
% not \gladd{complex enough for real-world scenarios}~\yscomment{We can say ``which is limited for real-world scenarios.''}. 
% To fill in this gap, \textbf{ComplexQuestions}~\cite{Bao-COLING-2016} dataset incorporated entity type, and temporal constraints to form complex questions. 

Different from simple questions which involve single fact reasoning on KB, existing work involves the following properties to construct complex KBQA questions:.
\begin{itemize}
	\item Multi-hop reasoning. Questions logically~\yscomment{``linearly''} composite multiple KB facts to reason on KB turn to be hard with large search space. 
	% For example, to reason answer for question ``Which person directed the movies starred by John Krasinski?'', we should first figure out the movies contain ``John Krasinski'' and then address their directors as the final answer.
	% (\eg composition type questions in ComplexQuestions).
	% ~\yscomment{Should we make it consistent to say it is ``multi-hop reasoning'' or ``multi-hop realtion'' or ``multi-hop fact''?}
	\item Constrained relations. Questions \jhadd{that} involve constraints (entity, temporal keywords) indicate we need to consider some constraint-involved relations to get the answer. For example, ``Which book did JK Rowling write in 1997'' queries about the relation with constraint ``1997''.
% 	~\yscomment{``Questions involve constraints (entity, temporal keywords) indicate we need to consider some constraint-involved relations to get the answer. For example, ``Which book did JK Rowling wrote in 1997'' queries about the relation with constraint ``1997''.''}  Take the question in Fig.~\ref{fig:example} as an example, ``TV producer'' is an entity type constraint.).~\yscomment{I feel it's better to give different and diverse examples.''}
	% (\eg conjunction type question in ComplexQuestions, temporal aspect question in LC-QuAD 2.0).~\yscomment{Still should we make it consistent to the ``constraint-involved realtions'' in the Introduction Section?}
	\item Numerical operations. Questions which require numerical operations to obtain answer (\eg counting, ranking operations for comparative and superlative questions) is also complex to solve. 
	To obtain answer for question in  Fig,~\ref{fig:example}, we should rank all possible candidates according to their marriage date after a series of reasoning steps to fullfill the constraint ``first''.
	%\item Logical forms. Complex question can be transformed into specific logic form $l$ (\eg SPARQL, query graph) with the consideration of the structured KBs. And then such logical forms can be executed against the KB to obtain the correct answers. Part of datasets generate such logical form with templates, and further incorporate expert to help correct such logical form. For example, the ground truth query graph to answer question in Fig.~\ref{fig:example} is annotated with thick red borders.
	%\item Natural language. Compared with questions generated with predefined templates, natural language questions written by human are more challenging to answer.~\yscomment{For this property, I'm not sure whether we should mention it here as to my best knowledge, not all complex KBQA dataset is manually created and also this is not the unique property of complex questions. Maybe we want to emphasis the complex questions have more complicated semantics and syntax.}
	% ComplexWebQuestions contains four compositionality types by generating composition questions (45$\%$ of the times), conjunctions (45$\%$), superlatives (5$\%$) and comparatives (5$\%$).
	% \item template or natural language. \eg, MetaQA is fully generated from templates.
\end{itemize}

%Despite complex questions properties, some other factors are taken into consideration when constructing the complex KBQA dataset. 
%Compared with questions generated with predefined templates, natural language questions written by human are more challenging to answer.
Many datasets begin with defining some templates which involve above complex question properties and then instantiate the templates with certain entities and relations in KB to generate questions.
Crowd workers are further employed to paraphrase the template-based questions.
The natural language questions paraphrased or directly written by human beings are more challenging to answer.
Generally, a complex question can be transformed into a logic form (\eg subgraph, query graph)\yscomment{Is it okay to mention ``query graph'' here without explanation as we plan to explain later?}.% with the consideration of the structured KBs. 
Such a logic form can be further mapped into an RDF query (i.e. SPARQL) which can be used to execute against a KB to retrieve the entities in KBs.
For example, the ground truth query graph to answer question in Fig.~\ref{fig:example} is annotated with thick red borders. 
Some complex KBQA datasets provide the annotations of the ground truth logic forms.
They generate such logical forms with templates and incorporate experts to help correct them manually. \yscomment{I slightly revised the paragraph to first talk about complex question generations then logic form annotations. I'm thinking whether we should change the title to ``Dataset Generation''.}

% \subsection{Dataset Descriptions}
% There have been a number of datasets collected for the complex KBQA task. We present their descriptions in the following and summarize the statistics of the datasets in Tab.~\ref{tab:datasets}.
% ~\yscomment{If we already have the overall organization introduction right under the Section title ``Dataset'', we may not need to repeatly have above paragraph.}
}
\ignore{
\glcomment{KB schema, CVT and related concepts. To modify here. How KB support query language (ontology, different design), how KBs differ from each other} 
Freebase is built on the notions of objects, facts, types, and properties~\cite{Thomas-WWW-2016}. Each Freebase object has a stable identifier called a “mid” (for Machine ID), one or more types, and uses properties from these types in order to provide facts. For example, the Freebase object for Barack Obama has the mid $/m/02mjmr$ and 
the type $/government/us\_president$ (among others) that allows the entity to have a fact with the property $/government/us\_president/presidency\_number$ and the literal integer “44” as the value. 
Freebase uses Compound Value Types (CVTs) to represent n-ary relations with $n > 2$, \eg values like geographic coordinates, political positions held with a start and an end date, or actors playing a character in a movie. CVT values are just objects, \ie they have a mid and can have types (although they usually only have the compound value type itself)~\cite{Thomas-WWW-2016}. 
Wikidata’s data model relies on the notions of item and statement. An item represents an entity, has a stable identifier called “qid”, and may have labels, descriptions, and aliases in multiple languages; further statements and links to pages about the entity in other Wikimedia projects—most prominently Wikipedia. Contrary to Freebase, Wikidata statements do not aim to encode true facts, but claims from different sources, which can also contradict each other, which, for example, allows for border conflicts to be expressed from different political points of view.
}

% \ignore{
~\glcomment{The following paragraphs describe relations between these benchmarks, not necessary, we may delete them and spend some space on resource part. To discuss.}
A series of research work follows \textbf{WebQuestions}~\cite{Berant-EMNLP-2013} to construct complex KBQA datasets, and these datasets become popular benchmarks. 
% In this study~\yscomment{The coreference is not clear here, how about ``Regarding WebQuestions''?},
% interrogatives to ask certain types of questions,
Regarding WebQuestions, Berant \etal~\cite{Berant-EMNLP-2013} used the Google Suggest API to obtain questions that begin with a \textit{wh}-word (\eg what, when and why) and contain exactly one entity, and obtain question-answer pairs from topic entity's Freebase page. 
However, most of questions in WebQuestions dataset only require single fact reasoning on KBs, which is not common enough for real-world scenarios.
% not \gladd{complex enough for real-world scenarios}~\yscomment{We can say ``which is limited for real-world scenarios.''}. 
To fill in this gap, \textbf{ComplexQuestions}~\cite{Bao-COLING-2016} dataset incorporates entity type, and temporal constraints to form complex questions. 
As WebQuestions provides only question-answer pairs, Yih \etal~\cite{Yih-ACL-2016} constructed \textbf{WebQuestionsSP} dataset through annotating SPARQL query statements for each question in WebQuestions.
% \gladd{"Furthermore", or "To guarantee question's correctness"}~\yscomment{I feel ``Furthermore'' is better.}
Furthermore, they removed questions with ambiguous expressions, unclear intentions, or invalid answers. 
% \gladd{To evaluate the idea of decomposing complex questions into a sequence of simple questions, ~\citeal{CWQ-NAACL-2018} collected \textbf{ComplexWebQuestions} dataset based on \textbf{WebQuestionsSP} dataset. 
% Based on the SPARQL queries from \textbf{WebQuestionsSP} dataset, ~\citeal{CWQ-NAACL-2018} create more complex queries that include phenomena such as function composition, conjunctions, superlatives and comparatives.}~\yscomment{I think pointing out this dataset is to evaluate the decomposing method may limit their purpose.}
% \yscomment{We can simply say ``\citeal{CWQ-NAACL-2018} collected \textbf{ComplexWebQuestions} dataset based on \textbf{WebQuestionsSP}.
% This dataset contain more complex questions that include query compositions, conjunctions, superlatives and comparatives, etc.''}
Talmor \etal~\cite{CWQ-NAACL-2018} collected \textbf{ComplexWebQuestions} dataset based on WebQuestionsSP.
This dataset contains more complex questions that include four types of query: composition, conjunction, superlative and comparative.

Question Answering over Linked Data (\textbf{QALD})~\cite{QALD} is a series of evaluation challenges on question answering over linked data. 
% ~\yscomment{Is ``challenge'' more commonly used to describe a competition? We can also provide the link of this challenge if it is available.} 
Since 2011, there have been nine challenge datasets released, including complex questions which contain multiple relations or subjects, questions with (time, comparative, superlative, and inference) constraints, and multilingual questions. 
% \gladd{However, \textbf{QALD} datasets are insufficient in terms of size, variety or complexity to apply and evaluate a range of machine learning based QA approaches for learning complex SPARQL queries.}~\yscomment{Before we introduce semantic parsing based methods, the readers may not understand why we need to learn SPARQL queries so it's better to avoid mention this.}~\yscomment{Can we say ``However, \textbf{QALD} datasets are insufficient in terms of size, language variety or complexity to apply and evaluate a category of machine learning based KBQA approaches.''}
However, \textbf{QALD} datasets are insufficient in terms of size, language variety or complexity to evaluate a category of machine learning-based complex KBQA approaches.
% To evaluate a range of machine learning based QA approaches for learning complex SPARQL queries, LC-QuAD 1.0~\cite{LC-QuAD-ISWC-2017} and LC-QuAD 2.0\cite{LC-QuAD-2.0-ISWC-2019} were constructed with larger size and varied complexity. 
To obtain complex questions with larger size and varied complexity, \textbf{LC-QuAD 1.0}~\cite{LC-QuAD-ISWC-2017} and \textbf{LC-QuAD 2.0}~\cite{LC-QuAD-2.0-ISWC-2019} are constructed with the following process: 
It begins by creating a set of SPARQL templates, a list of seed entities, and a relation whitelist. 
Then 2-hop subgraphs are extracted for each seed entity from target KBs considering applicable relations. And valid SPARQL queries can be grounded with facts in the subgraph. 
Finally, these template queries are converted to natural language questions through predefined question templates and crowdsourcing. 
% \yscomment{What's the function of predicate whitelist here?}~\glcomment{I checked the LC-QuAD 2.0 dataset paper\cite{LC-QuAD-2.0-ISWC-2019}: for every sparql template only a part of predicates are selected to build SPAQL. So I think it was only used to constrain the sparql generation.}
While LC-QuAD 1.0 uses DBpedia as its knowledge resource, LC-QuAD 2.0 chooses both DBpedia and Wikidata.
% While \textbf{LC-QuAD 1.0} use\yscomment{``uses''} single DBpedia as the target KB, \textbf{LC-QuAD 2.0} further introduce popular KB Wikidata\yscomment{This sentence makes readers misunderstand they introduced KB Wikidata, we can say ``While \textbf{LC-QuAD 1.0} uses DBpedia as its knowledge resource, \textbf{LC-QuAD 2.0} chooses Wikidata.''}.

% Besides popular benchmarks, recently some large-scale datasets are constructed to foster researches on complex KBQA.\glcomment{This paragraph describes four large scale datasets. But I think they are relatively independent. Should we just ignore these new datasets? As survey of Qiu \etal don't mention them.}~\yscomment{I think introducing them is a good thing for us as we do it more comprehensively. 
% Also it maybe not suitable for us to say ``Besides popular benchmarks'' as this indicates the other datasets are not ``popular'', we can say ``Besides above benchmarks, recently, more large-scale datasets are constructed to foster researches on complex KBQA.''}
Besides the above benchmarks, recently, more large-scale datasets are constructed to foster researches on complex KBQA.
\textbf{MetaQA Vanilla}~\cite{Zhang-AAAI-2018} dataset contains more than 400k single and multi-hop (up to 3-hop) questions in the domain of movie, which is a comprehensive extension of WikiMovies~\cite{KVMem-EMNLP-2016} with manual defined templates.
\textbf{CFQ}~\cite{CFQ-ICLR-2020} is a simple yet authentic and large natural language understanding~(NLU) dataset that is initially designed to measure models' compositional generalization capability. 
It contains 239,357 English question-answer pairs that are answerable using the public Freebase data. 
Besides, it also provides each question with a corresponding SPARQL query against the Freebase.
% Recently, \citeal{KQA-Pro} released a large-scale dataset \textbf{KQA Pro}~\cite{KQA-Pro} for Complex KBQA. 
% They proposed compositional strategies to generate questions, corresponding SPARQLs, and Programs (which represent reasoning process)\yscomment{Can you paraphrase this sentence as it's hard to understand?} with a small number of templates, and then paraphrase the generated questions to natural language questions by crowdsourcing.
% The question generation can be divided into two stages: locating and asking. In locating stage a single entity or an entity set with various restrictions are located with predefined rules, while in asking stage query specific information about the target entity or entity set is generated through templates. When generating textual snippet from template, they also generate the snippet of logical forms (\eg SPARQL) using corresponding rules. And finally the generated questions are paraphrased to natural language questions by crowdsourcing.~\glcomment{I am a little confused here. Do you think it make sense to describe the construction process for this dataset?}
% Recently, \citeal{KQA-Pro} released a large-scale dataset \textbf{KQA Pro}~\cite{KQA-Pro} for Complex KBQA. 
\textbf{KQA Pro}~\cite{KQA-Pro} is a large-scale dataset for complex KBQA, which contains around 120,000 diverse questions paired with corresponding SPARQLs. 
% Besides SPARQL, Shi \etal~\cite{KQA-Pro} defined a compositional and highly interpretable formal format, named \textit{Program}, to represent the reasoning process of complex questions.~\yscomment{``define'' could easily make people misunderstand the program is the novelty of this paper, how about ``provided \textit{Program} annotations to data, which is a compositional and highly interpretable formal format to represent the reasoning process of complex questions.''}
Besides SPARQL, Shi \etal~\cite{KQA-Pro} provided \textbf{\textit{Program}} annotations to data, which is a compositional and highly interpretable format to represent the reasoning process of complex questions.
% ~\glcomment{I delete some contents to make it compact.}
% Through compositional strategies, questions, corresponding SPARQLs, and Programs are generated with a small number of templates. 
% And the generated questions are paraphrased to natural language questions by crowdsourcing.
While most prior work followed i.i.d. assumption to construct complex KBQA dataset, Gu~\etal~\cite{GrailQA-2020} argued that i.i.d. may be neither reasonably achievable nor desirable on large-scale KBs.
% \ysadd{Unsatisfied data distribution commonly occurs in real scenarios.} 
Out-of-distribution data occurs frequently in real-world scenarios and existing methods are rarely evaluated under such challenging settings. 
To fill in this gap, they built a complex KBQA dataset \textbf{GrailQA} with three levels of built-in generalization: i.i.d., compositional, and zero-shot.
